Non-contact Lung Disease Classification via OFDM-based Passive 6G ISAC Sensing

This paper is the first to present a novel, non-contact method that utilizes orthogonal frequency division multiplexing (OFDM) signals (of frequency 5.23 GHz, emitted by a software defined radio) to radio-expose the pulmonary patients in order to differentiate between five prevalent respiratory diseases, i.e., Asthma, Chronic obstructive pulmonary disease (COPD), Interstitial lung disease (ILD), Pneumonia (PN), and Tuberculosis (TB). The fact that each pulmonary disease leads to a distinct breathing pattern, and thus modulates the OFDM signal in a different way, motivates us to acquire OFDM-Breathe dataset, first of its kind. It consists of 13,920 seconds of raw RF data (at 64 distinct OFDM frequencies) that we have acquired from a total of 116 subjects in a hospital setting (25 healthy control subjects, and 91 pulmonary patients). Among the 91 patients, 25 have Asthma, 25 have COPD, 25 have TB, 5 have ILD, and 11 have PN. We implement a number of machine and deep learning models in order to do lung disease classification using OFDM-Breathe dataset. The vanilla convolutional neural network outperforms all the models with an accuracy of 97%, and stands out in terms of precision, recall, and F1-score. The ablation study reveals that it is sufficient to radio-observe the human chest on seven different microwave frequencies only, in order to make a reliable diagnosis (with 96% accuracy) of the underlying lung disease. This corresponds to a sensing overhead that is merely 10.93% of the allocated bandwidth. This points to the feasibility of 6G integrated sensing and communication (ISAC) systems of future where 89.07% of bandwidth still remains available for information exchange amidst on-demand health sensing. Through 6G ISAC, this work provides a tool for mass screening for respiratory diseases (e.g., COVID-19) at public places.

==> Figures/abstract.tex <==
\begin{abstract}

This paper considers an Internet of Things (IoT) blockchain network consisting of a leader node and various follower nodes which together implement the RAFT consensus protocol to verify a blockchain transaction, as requested by a blockchain client. Further, two kinds of active attacks, i.e., jamming and impersonation, are considered on the IoT blockchain network due to the presence of multiple {\it active} malicious nodes in the close vicinity. When the IoT network is under a jamming attack, we utilize the stochastic geometry tool to derive the closed-form expressions for the coverage probabilities for both uplink and downlink IoT transmissions. On the other hand, when the IoT network is under the impersonation attack, we propose a novel method that enables a receive IoT node to exploit the pathloss of a transmit IoT node as its fingerprint to implement a binary hypothesis test for transmit node identification. To this end, we also provide the closed-form expressions for the probabilities of false alarm, missed detection, and miss-classification. Finally, we present detailed simulation results that indicate the following: i) the coverage probability improves as the jammers' locations move away from the IoT network, ii) the three error probabilities decrease as a function of the link quality.
\\
\end{abstract}



==> Figures/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This paper studied active (jamming and impersonation) attacks on a RAFT-based IoT blockchain network. The impact of the jamming attack on the IoT blockchain network was evaluated via coverage probability analysis for both uplink and downlink IoT transmissions. On the other hand, the impersonation attack on the IoT blockchain network was countered by means of a novel, physical-layer method that exploited the pathloss of a transmit IoT node as its fingerprint to construct a binary hypothesis test for transmit node identification. To this end, closed-form expressions were provided for the probabilities of false alarm, missed detection, and miss-classification. Simulation results showed that for the jamming attack, an increase in the threshold value reduces the coverage probability and high intensity of jammers produces low coverage probability, while for the impersonation attack, pathloss can be used as device fingerprint and above $95 \%$ of detection probability can be achieved  with a minimum of $0.1$ false alarm for a $10$ dB link quality.

==> Figures/keywords.tex <==
\begin{keywords}

Effective capacity, D2D communication, Overlay, Inband, 5G

\end{keywords}} 

==> Figures/sec1.tex <==
\section{Introduction}
\label{sec:intro}

 The next generation wireless networks are supposed to have support for processing at the edge, automation, and distributed trust, which can be accomplished using blockchain-enabled wireless networks \cite{Zhang:IWC:2021}.
  Blockchain  technology has great capability in wireless networks (specifically, Internet of thing (IoT) devices) for  developing trust and consensus procedures without the intervention of a central party \cite{nguyen2019blockchain}. Recently, some prominent works are reported in the literature studying blockchain-based wireless networks. For the first time, Y.Sun in \cite{sun2019blockchain} studies the wirelessly connected blockchain system where he provides optimal nodes deployment and relation of communication and transaction throughput. Further, the work \cite{xu2020raft} studies the security aspects of RAFT-based wireless networks with the presence of single jammer and derives the probability of achieving successful blockchain transactions via exploiting probability theory. Next, authors in \cite{Zhang:ICC:2020} maximize the transaction uploading and revenue of miners using the Stackelberg game approach in blockchain-based wireless networks. Following \cite{xu2020raft}, authors in \cite{zhuz2020blockchain} provide theoretical calculation of required throughput and transmission successful probability to support the system.  Further Hao in his perspective article \cite{Hao:DCN:2020} discusses the potentials of blockchain for resource management in 6G. Particularly, he discusses  device-to-device, IoT, and network-slicing applications of 6G for resource management.
  More recently, \cite{zhang2:arXiv:2021} answer the question that how many resources are needed to run wireless blockchain networks. Particularly, the impact of the provision of resources is studied on the performance of blockchain. Dynamic spectrum sharing is studied in  \cite{Liu:IWCMC:2021}, where reinforcement learning is utilized to analyze the resource-sharing structure and spectrum-sharing process in a blockchain system combined with 6G hybrid cloud. Next, the authors in \cite{Xuefei;IOTJ;2021} study the block propagation in blochchain-based vehicular ad-hoc networks. They study the dynamic of block propagation and provide a closed-form expression for block propagation time. The work \cite{Hou:ICL:2021} minimizes the latency in storing data by intelligent transaction migration policy by exploiting the Markov process and deep deterministic policy gradient. The authors in \cite{Li:TVT:2021} focus on blockchain-based wireless local area networks and provide a new medium access control protocol known as block access control. Specifically, its design is studied with, modeling and analyses. Finally, the authors in \cite{Hao:Arxiv:2021} propose Blockchain Enabled Radio Access Network (BE-RAN). They provide a security framework for mutual authentication based on digital signatures/secret keys. They also provide design guidelines for switching, routing, and quality of service management.
  %There is no dense research on the emerging wireless blockchain network, so there is some concern that needs to be addressed. Recently  developed the Blockchain-enabled IoT network. Using his theory, Hao Xu  showed that RAFT-based consensus protocol could be a feasible solution for blockchain under the circumstance of IoT ecosystems. In that scheme, all the nodes (client, leader, and follower) of the private blockchain are wirelessly connected, and no Byzantine node was allowed, so failure is only due to communication link. The author tried to analyze the security perspective in terms of transaction success rate in the presence of a single jammer. The transaction success rate depends on both communication methods (leader to follower and follower to leader). Communication drop from 50\% cause to fail the consensus. So, in the Raft-based mechanism, the consensus is achieved if and only if the leader gets at least 51\% majority.

  
  %between the users as it does not involve the third party or centralized authority. New opportunities are created by integrating blockchain with IoT to empower IoT and blockchain services and applications. Blockchain act as a distributed ledger whose data represents a list of transactions between a few banks or the conversation between a few parties
 The ground basis of blockchain is the consensus techniques that establish trust and update the ledger's states which can be broadly  classified into two classes \cite{nguyen2018survey}. The first class, which is based on pure computation, solves the mathematical puzzle by joining nodes of the blockchain network to prove that they are eligible for mining work, e.g., Proof-of-Work (PoW) \cite{peer} and Proof of Stacks (PoS) \cite{vasin2014blackcoin}. The second class relies on pure communications between joining nodes. The successful voting of majority nodes through the communication channel leads to the achievement of consensus, i.e. Byzantine Fault Tolerance (BFT) \cite{castro1999practical}, Paxos \cite{lamport2019part}, and RAFT \cite{ongaro2014search}. Private blockchains use second class due to their low complex nature, high throughput and small confirmation delay \cite{dinh2018untangling}. Low-complex consensus techniques might be used in wirelessly connected IoT devices to develop the distributed system. Primary implementations of consensus in the private blockchain were based on Paxos over the last decade. Unfortunately, it is not easy to understand due to its intricate architecture, and aloof nature for practical systems. Therefore, a new consensus protocol (so-called RAFT) was developed that has a concise definition and comparable performance. 
 RAFT reduces the degree of non-determinism by decomposing the nodes into two types of roles, one leader and the others are follower nodes. \textcolor{black}{ In such a network, blockchain consensus protocol will fail if follower nodes do not cast their votes due to communication failure or dishonest votes cast by malicious actors \cite{xu2020raft}.}
%  RAFT implements the consensus by first electing a leader that receives log entries/transaction details from the client. The leader has the responsibility to manage the new log entries and replicate them on the servers. In contrast, followers are passive nodes that only respond to the request of the leader. The leader can only be replicate the logs on servers when the majority of followers successfully vote back to the leader \cite{ongaro2014search}. 


 
 
%{\bf Motivation \& Contribution}: 
%Traditionally wired network is employed for blockchain because wired channels are more stable and secure. However, blockchain development in


Blockchain technology serves as securing different IoT applications, but it is also vulnerable to different attacks \cite{ferrag2018blockchain}. These attacks on the blockchain systems lead to the failure of the consensus process responsible for verifying the transactions in the blockchain. 

This work studies two types of active malicious attacks: jamming attacks and impersonation attacks in a RAFT-based blockchain system. The coverage probability is derived in order to assess the impact of jamming in uplink and downlink transmissions. 


On the other hand, physical layer authentication to counter impersonation attacks is an emerging domain in the field of information security \cite{aman2022security}.  Recently, to counter the impersonation attacks at the physical layer, \cite{Aman:Access:2018} and \cite{waqas:ICC:2020} propose distance, angle of arrival and position, \cite{Ammar:VTC:2017} and \cite{Aman:UCET:2019} propose channel impulse response, and  \cite{Aman:UCET:2020} exploits the lack of hardware reciprocity as features or device fingerprints to carried out authentication. We in this work encountered impersonation attacks by exploiting the pathloss of the transmitter nodes.

{\bf Contributions.} This work considers a RAFT-based IoT blockchain network that comprises a leader node and many follower nodes which together verify a blockchain transaction upon request from a blockchain client. To the best of the authors' knowledge, this work is the first that considers the two most prominent kinds of active attacks (jamming and impersonation) on the IoT blockchain networks. Specifically, two main contributions of this paper are as follows:
\begin{itemize}
    \item When the IoT blockchain network is under jamming attack, we utilize the stochastic geometry tool to derive the coverage probabilities for both uplink and downlink IoT transmissions, as a function of important system parameters, e.g., transmit power of legitimate and jamming nodes, intensity and relative geometry of the jamming nodes, etc. 
    \item When the IoT blockchain network is under impersonation attack, we propose a novel counter-method that enables a receive IoT node to exploit the pathloss of a transmit IoT node as its fingerprint to construct a two-step testing approach (i.e. Maximum Likelihood test followed by the binary hypothesis test). Furthermore, we provide closed-form expressions for the three error probabilities of interest, i.e., false alarm, missed detection and miss-classification.
\end{itemize}

{\bf Outline.} The rest of this paper is organized as follows. Section II provides a detailed description of the considered system model. Section III considers the scenario of a jamming attack on the IoT blockchain network, and derives the coverage probability for both uplink and downlink IoT transmissions. Section IV considers the scenario of an impersonation attack on the IoT blockchain network, and presents a novel countermeasure that enables a receive IoT node to exploit pathloss as a fingerprint of a transmit IoT node to implement a hypothesis testing test for transmitter identification. Section V provides simulation results. Finally, Section VI concludes the paper.

{\bf Notations.} Unless specified otherwise, $\vert.\vert$ and $\Vert.\Vert$  denote the modulus and the 2-norm respectively, $\mathbb{E}(.)$ is the expectation operator, boldface letters such as $\mathbf{X}$ represents a vector and $\mathcal{CN}$ means complex normal.
\begin{figure}[htp]
    \centering
    \includegraphics[width=6cm]{Updated_system_final1.jpg}
    \caption{System Model}
    \label{fig:sys}
\end{figure}



==> Figures/sec2.tex <==

 \section{System Model \& Background}
\label{sec:sys-model}

\subsection{System Model}	
The IoT blockchain network based on the RAFT consensus algorithm comprises two parts, a wireless consensus network, and IoT clients, as shown in Fig. \ref{fig:sys}. The two parts may or may not be geographically isolated. The figure illustrates the communication
network topology and the IoT nodes' roles interchangeably in different business models. Any IoT node in the network can play a client's role that sends out transaction-requests or a leader/follower in the consensus process. The followers and malicious nodes' locations in a 2-Dimensional free space are modeled as Poisson Point Process (PPP)  and the leader (full node) is fixed at the geo-center of the consensus network. We consider that malicious nodes are  active malicious nodes who are capable of launching jamming and impersonation attacks. We assume that malicious nodes either launch jamming attacks or impersonation attacks in a given time. \\
\textcolor{black}{In jamming mode, malicious nodes continuously transmit noise/jamming signals in the available spectrum of communication for both uplink and downlink transmissions in order to destroy the voting process in IoT wireless blockchain networks. Thus, it is critically important to explore the blockchain transactions success rate in the form of coverage probability in the presence of radio jamming \cite{xu2020raft}. On the other hand, in impersonation mode, the malicious nodes aim to represent themselves as legitimate nodes and cast votes to select a leader. Therefore, it is important to counter impersonation attacks by using a physical layer authentication mechanism.   }

\subsection{RAFT Consensus Protocol}
\textcolor{black}{ RAFT consensus algorithm begins by first electing a leader who receives log entries/transaction-details from the client. The leader has high capabilities such as better performance and reliability to manage the new log entries and replicate them into the blockchain. In contrast, followers are passive nodes that only respond to the request of the leader. The leader can only insert the transaction-details into the blockchain when most followers successfully vote back to the leader.
The RAFT consensus mechanism is triggered as follows. Firstly, the leader receives the transaction information from clients and performs some necessary actions to form a block. Secondly, a leader will communicate with follower nodes via a downlink (DL) broadcasting channel to approve the block. When followers successfully received a DL message, they verify and send the voting message on the multi-access uplink (UL) channel for confirmation. Lastly, a leader will count the vote to achieve consensus; if the leader gains the majority more than 50\%  from the followers (voters).}

This paper focuses on communication inside the consensus network, on both DL and UL. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \section{Jamming Attack on IoT Blockchain Network}
\label{sec:Jamming}



In the RAFT consensus algorithm, a client transmits transaction requests to the leader node to make consent with the followers by considering that all follower nodes are honest. % \textcolor{red}{However, malicious nodes can exist in the network due to the wireless channel's openness which prevents consensus from being achieved among the nodes through spectrum jamming. These jammers are not part of the consensus network and cannot cast votes. However, they transmit radio signals that disrupt communications among the leader and honest/follower nodes by decreasing the signal-to-noise ratio. Thus, it is critically important to explore the blockchain transactions' success rate in the presence of radio jamming \cite{xu2020raft}.} 
This section finds success/coverage probability defined as receiving Signal to Interference and Noise Ratio (SINR) is greater than its predefined threshold between a leader and associated follower. All followers operate in the same frequency band, so they cause increased interference that ultimately degrades the received SINR and lowers the success probability. Different protocols were employed in the private blockchain networks to avoid interference and collision among the follower nodes, such as centralized radio resource allocation and Carrier Sense Multiple Access (CSMA) or transmission interval made large enough so that collision is negligible.
\subsection{Coverage Probability for IoT Transmissions on the Downlink}
\label{sec:Downlink}

When the leader transmits, then a typical follower receives the following baseband signal:
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation} 
\label{eq:y}
y = \sqrt{P} Hs + \sum_{j\in\phi_{J}} \sqrt{P_j} H_j s + n,
\end{equation}
where $P$ ($P_j$) is the transmit power of the leader ($j$-th jammer) node, $s$ is the transmitted symbol, $H=h/\sqrt{R^\alpha}$ ($H_j=h_j/\sqrt{R_j^\alpha}$) represents the wireless propagation from the leader (jammer) to the follower, and $R$ ($R_j$) is the random distance between the leader (jammer) and the follower node. Further, for the leader-follower link, $R^{-\alpha}$ is the large-scale fading/pathloss component, ${\alpha}$ is the pathloss exponent, $h \sim \mathcal{CN}(0,1)$ is the small-scale fading component. Moreover, $\sqrt{I_{J}} =\sum_{j\in\phi_{J}} \sqrt{P_j} H_j s$ is the aggregate interference amplitude due to multiple jammers where $\phi_{J}$ indicates that the jammers are distributed in a 2-dimensional free-space as PPP. Finally, \textcolor{black}{$n \sim \mathcal{CN}(0,\sigma^2)$ is the additive white Gaussian noise with power $\sigma^2$.}

We consider an interference-limited scenario (i.e., the interference is much larger than the noise). This allows us to consider the signal-to-interference ratio (SIR) as the performance metric. The SIR of a typical follower associated with the leader node is given as:  

\begin{equation}
\label{eq:SIR}
SIR^{DL}=\dfrac{P|h|^2{R^{-\alpha}}}{I_J},
\end{equation}
where $I_{J}=\sum_{j\in\phi_{J}}{P_{j}}|h_j|^2{\Vert\mathbf{X}_j\Vert^{-\alpha}}$ is the aggregate interference power, $h_j\sim \mathcal{CN}(0,1)$ is the small-scale fading component on the jammer-follower channel, and $\mathbf{X}_j$ is the random location of $j$-th jammer or Poisson point (note that $\Vert\mathbf{X}_j\Vert=R_j$). 
	
The IoT transmission from the leader to any given follower node on the DL will be considered successful only when the received SIR is greater than a pre-specified threshold $\beta_D$ \cite{lu2021stochastic}. Thus, the transmission success probability, or, the coverage probability for the DL ($\mathcal{P}^{DL}_c$) is defined as follows:
\begin{equation}
\label{eq:hh}
    \mathcal{P}^{DL}_c(\alpha,\beta_D)= \mathcal{P}\biggl[SIR^{DL}>\beta_D\biggl]=\mathcal{P}\biggl[\dfrac{P|h|^2{R^{-\alpha}}}{I_{J}}>\beta_D\biggl].
\end{equation}


Now, we assume that a typical follower is at distance $r$ from the leader, then the coverage probability can be expressed as:
\begin{equation}
\label{eq:Pdl}
    \mathcal{P}^{DL}_c(\alpha,\beta_D)= \mathbb{E}_{R} \biggl[\mathcal{P}\biggl[SIR^{DL}>\beta_D \mid R=r\biggl]\biggl],
\end{equation}
\begin{equation}
=\int_{r>0}^\infty \mathcal{P}\biggl[SIR^{DL}>\beta_D \mid r\biggl]f_R(r)dr, \nonumber
\end{equation}
where $f_R(r)$ is the probability density function (PDF) of $R$, and  is given as \cite{Mathai1999AnIT} \footnote{We consider the elected leader node at the origin of considered space}: 
\begin{align}
f_R(r)=2\pi\rho r \exp({-\rho \pi r^2}), 
\end{align}
\textcolor{black}{where $\rho$ is the intensity/density of the IoT nodes.} At this stage, first we need to compute $\mathcal{P}\big[SIR^{DL}>\beta_D \mid r\big]$ which can be expressed as:
\begin{equation}
\mathcal{P}\biggl[SIR^{DL}>\beta_D \mid r\biggl] = \mathcal{P}\biggl[|h|^2>\dfrac{{r^{\alpha}}\beta_D }{P} I_{J}\biggl]. 
\end{equation}
As $|h|^2\sim \exp(1)$, we can write: 
\begin{equation}
\mathcal{P}\biggl[|h|^2>\dfrac{{r^{\alpha}}\beta_D }{P} I_{J}\biggl] = \mathbb{E}_{I_J}\biggl[\exp(-\dfrac{{r^{\alpha}}\beta_D }{P} I_{J})\biggl]=\mathcal{L}_{I_{J}}(\dfrac{{r^{\alpha}}\beta_D }{P}),
\end{equation}
    where $\mathcal{L}_{{I}_{J}}(s)$ denotes the Laplace transform of the aggregate interference $I_{J}$ which is computed in Appendix A (with variable $s=\dfrac{{r^{\alpha}}\beta_D }{P}$).
%where $P_{L}$ is the transmit power of the leader,
%$h_l$ is the  channel between the leader and the follower, and $r_l$ is the distance between the leader and the follower. Next step is not always computed because the PDF of the jamming interference $I_{J}$ is not available in closed-form except for exceptional cases. However, complementary CDF of SIR can be expressed in terms of the Laplace transform (LT) of $I_J$ if and only if $|h|^{2}$ is exponentially distributed \cite{7733098}:
%\begin{equation}
%\mathcal{P}^{DL}(\beta_D)=E_{r_{l},I_{J}}\biggl[exp(-\dfrac{{r_{l}^{\alpha}}\beta_D }{P_{L}} I_{J})\biggl]
%\end{equation}
%let $s=  {{r_{l}^{\alpha}}\beta_D }/{P_{L}}$ and rewrite the above equation using the laplace definition as:

%\begin{equation}
%P^{DL}(\beta_D)= E_{r_{l}}[E_{I_{J}}exp(-s I_{J})]=E_{r_{l}}[\mathcal{L_{I_{J}}}(s)]
%\end{equation}

%%%%
%Given that leader is located at the  geo-center of consensus network having density $\rho_L$  and distance among the trusted follower is $r_l$, PDF of distance from the  leader is according to the Proposition $1$ in \cite{sun2019blockchain} given as: 
%\begin{align}
%f(r_l)=2\pi\rho_L r_l  exp({-\rho_L \pi r_l^2})   
%\end{align}

%The DL success probability expression, $P^{DL}(\beta_D)$, for leader, while considering PPP distribution of jammers, can be written as:
%\begin{align}
%P^{DL}(\beta_D)=\int_{r_l\geq 0}\mathcal{L_{I_{J}}}(s) f(r_l)dr_l
%\end{align}
% Where $\mathcal{L_{I_{J}}}(s)$ is computed in Appendix. 
Putting back the result of Appendix A to Eq. \ref{eq:Pdl} we get the following final expression of coverage probability for DL: 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%
\begin{equation}
\begin{split}
& \mathcal{P}^{DL}_c(\alpha,\beta_D)={2\pi\rho}\bigintsss_{r\geq 0}\exp\biggl(\dfrac{\pi \rho_J \gamma_{j}\beta_D r^{\alpha}}{(\alpha/2)-1} 
    \biggl[z_2^{(2-\alpha)}\\
    &{}_{2}F_{1}(1,1-{\dfrac{2}{\alpha}},2-{\dfrac{2}{\alpha}},-\gamma_J \beta_D (\dfrac{r}{z_2})^\alpha)-z_1^{(2-\alpha)}\\
    &{}_{2}F_{1}(1,1-{\dfrac{2}{\alpha}},2-{\dfrac{2}{\alpha}},-\gamma_J \beta_D         (\dfrac{r}{z_1})^\alpha)\biggl]-\rho \pi r^2 \biggl) r dr.
\end{split}
\end{equation}

  %%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsection{Coverage Probability for IoT Transmissions on the Uplink}
\label{sec:Uplink}
To achieve the consensus, followers send the voting message on the multi-access UL channel for confirmation after receiving a DL message. Consensus will be achieved if more than  $50\%$  from the followers successfully verify the transaction on the UL channel. So, we need to compute the success probability on the UL channel. We assume that CSMA is the medium access technique adopted by the followers and transmission on UL is available all the time (i.e., no idle channel). Then the coverage probability for a typical follower node on the UL is given as  \cite{lu2021stochastic}:
\begin{equation}
\mathcal{P}^{UL}_c(\alpha,\beta_U)=\mathcal{P}\biggl[SIR^{UL}>\beta_U\biggl]=\mathcal{P}\biggl[|h^{U}|^2>\dfrac{{R_{U}^{\alpha}}\beta_U }{P_{F}} I_{J}^{U}\biggl],
\end{equation}
where $\beta_U$ is a predefined threshold for UL, $h^{U}$ is the channel gain and $R_{U}$ is the distance from a typical follower to the leader on UL, $P_F$ is the transmit power of a typical follower,  and  $I_{J}^{U}$ is the aggregated interference to the leader.
CSMA makes sure no interference from the other follower nodes on the UL and hence the interference/jamming is due to the jammers only. This makes the coverage probability formulation the same as we do for DL.
We compute UL success probability using the same procedure as above, and we get:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{split}
&   \mathcal{P}^{UL}_c(\alpha,\beta_U)={2\pi\rho}\bigintsss_{r\geq 0}\exp\biggl(\dfrac{\pi \rho_J \gamma_{j}^U\beta_U r_{U}^{\alpha}}{(\alpha/2)-1} 
    \biggl[z_2^{(2-\alpha)}\\
    &{}_{2}F_{1}(1,1-{\dfrac{2}{\alpha}},2-{\dfrac{2}{\alpha}},-\gamma_j^U \beta_U (\dfrac{r_{U}}{z_2})^\alpha)-z_1^{(2-\alpha)}\\
    &{}_{2}F_{1}(1,1-{\dfrac{2}{\alpha}},2-{\dfrac{2}{\alpha}},-\gamma_j^U \beta_U         (\dfrac{r_{U}}{z_1})^\alpha)\biggl]-\rho \pi r_{U}^2 \biggl) r_{U} dr_{U},
\end{split}
\end{equation}
where $\rho_J$ is the intensity of jammer nodes and $\gamma_{j}^U ={P_{j}}/{P_{F}}$.

\subsection{Overall Coverage Probability}
\label{sec:joint}
Consensus is achieved when followers successfully receive the leader's request to verify the transaction-detail over the DL channel and respond to the leader over the UL channel. So, we derive the joint coverage probability in an IoT blockchain network as follows
\cite{7343565}:

\begin{equation}
    \mathcal{P}_{c}={\mathcal{P}[SIR^{UL}>\beta_U]}.{\mathcal{P}[SIR^{DL}>\beta_D]}
\end{equation}

\section{Impersonation Attack on IoT Blockchain Network}

In the RAFT consensus algorithm, due to the broadcast nature of wireless communication, the consensus algorithm may be failed due to the impersonation attacks launched by nearby malicious/illegitimate node(s) (so-called Eve(s)). In impersonation attacks, malicious nodes try to claim themselves as legitimate nodes/followers by utilizing a forged character in order to destroy the consensus mechanism. 


In this work, we provide a physical layer authentication mechanism to counter impersonation by illegitimate nodes. 
We, in this work, exploit the pathloss of the transmitter node as a device fingerprint to counter the impersonation.  
%Thus, the success rate of the blockchain transactions in impersonating nodes is a critically important topic.   
 We assume a realization\footnote{Typically, in physical layer authentication, one needs to know the exact number of transmitting nodes in order to evaluate its performance. Therefore, in this part, we take a single realization of PPP in order to fix the total number of nodes (both, malicious and legitimate).} of PPP, specifically, $M$ follower (legitimate) nodes $\{F_i\}^{M}_{i=1}$ and $N$ Eve (malicious/illegitimate) nodes $\{E_j\}^N_{j=1}$ are considered in  a 2-Dimensional space, and a leader is placed at the center of the considered region. We assume that the transmitter nodes transmit with a fixed transmit power so that the leader can compute the pathloss. We also assume that the malicious nodes are transmitting with the same transmit power in order to stay stealth in the region \footnote{High power transmission will easily identify the transmitter as a malicious node. To get success in impersonating the legitimated nodes, malicious nodes transmit with the same power as legitimate nodes do}. The pathloss $\Psi$ in dB of a transmitter at the distance $d$ from the receiver is given as: 


\begin{align}
\label{eq:THzPL}
\Psi[dB]=10 \alpha \log_{10}(d),
\end{align}
where $\alpha$ is the pathloss exponent.



\subsection{The Proposed Authentication Method}
We assume that CSMA is the approach used by the followers and malicious nodes to cast their votes. We assume that malicious node $E_j$ could cast a vote, pretending to be a legitimate follower node when the channel is completely idle by the followers and hence, no collision. The leader is supposed to authenticate each received casting vote and correctly achieved the consensus. Furthermore, we assume that the leader already has the ground truths of legitimate nodes which he gets via prior training on a secure channel. The ground truth vector can be denoted by $\mathbf{\Psi} = \{\Psi_1, ..., \Psi_M\}^T$. As discussed earlier, we will authenticate the transmitter based on the pathloss feature. So the noisy measurement of pathloss $z = \Psi + n$ at a given time-slot is obtained by using the pulse-based method, where $\Psi$ is the pathloss and $n \sim \mathcal{N}(0,\sigma^2)\,$ is the noise/estimation error.  To counter the impersonation by malicious nodes, we first do a Maximum Likelihood (ML) test as follows: 

\begin{equation} 
\label{eq:ML}
i^* = \underset{i}{\max} \quad f(z\mid \Psi_i),
\end{equation}
where $f(z\mid \Psi_i)$ is the likelihood function or conditional PDF.\\
Equivalently, we can write \ref{eq:ML} as:

\begin{equation} 
\label{eq:ML-pl}
(TS^*,i^*) = \underset{i}{\min} \quad |z-\Psi_i|,
\end{equation}
where $TS^*$ is the minimum value of test statistics and $i^*$ returns the index of the transmitter node which is decided through ML. Next, we decide on impersonation through binary hypothesis testing as follows:

\begin{equation}
	\label{eq:H0H1}
	 \begin{cases} H_0 (\text{no impersonation}): & TS^*=\underset{i}{\min} |z(t)-\Psi_i| < \epsilon \\ 
                   H_1 (\text{impersonation}): & TS^*=\underset{i}{\min} |z(t)-\Psi_i| > \epsilon \end{cases},
\end{equation}
where $\epsilon$ is a small test threshold and is a design parameter that decides a vote from the node is accepted or not. 
Equivalently, we have:
\begin{align} 
\label{eq:bht}
{TS}^* \gtrless_{H_0}^{H_1} {\epsilon}.
\end{align}

The hypothesis
$H_0$ inferred that the legitimate node transmits the vote. Alternatively, the hypothesis $H_1$ implies that an illegitimate node transmits a vote. 
Further, we present closed-form expressions for the error probabilities. We have three types of errors resulting from the above tests. \textcolor{black}{These errors are: false alarm, missed detection, and miss-classification.
The probability of false alarm ($\mathcal{P}_{fa}$) is the probability that a legitimate follower casts a vote, but the leader identifies it as a malicious node. The probability of missed detection ($\mathcal{P}_{md}$) is the probability that a malicious node casts a vote, but the leader identifies it as a vote of a legitimate node. Last, the probability of miss-classification ($\mathcal{P}_{mc}$) is the probability that when no impersonation is detected but a wrong transmitter node is decided among the legitimate transmitters.}

We, in this work, follow the Neyman-Pearson lemma \cite{923720} where $\epsilon$ test threshold for a pre-defined false alarm $\mathcal{P}_{fa}$ can be chosen such that missed detection probability $\mathcal{P}_{md}$ is minimized. Thus, the error probabilities for the above hypothesis tests are:
\begin{equation}
\begin{split}
\mathcal{P}_{fa} &= \mathcal{P}(H_1|H_0)= \sum_{i=1}^M \mathcal{P}(TS^*>\epsilon|F_i)\pi (i) \\
&=\sum_{i=1}^M 2Q(\frac{\epsilon}{\sigma})\pi (i)=2Q(\frac{\epsilon}{\sigma})\sum_{i=1}^M \pi (i)=2Q(\frac{\epsilon}{\sigma})
\end{split}
\end{equation}
Where $\pi (i)$ is the prior probability of legal node  $F_i$ (we consider equal priors in our work), and $Q(x)=\frac{1}{\sqrt2\pi}\int_x^\infty e^{\frac{-t^2}{2}}dt$ is the complementary CDF of a standard normal distribution  Thus, the threshold could be computed as follows:

\begin{equation}
\label{eq:epsi}
\epsilon = \sigma Q^{-1}(\frac{\mathcal{P}_{fa}}{2})
\end{equation}

\subsection{The Performance of the Proposed Method}

Next, $\mathcal{P}_{md}$ is given as:
\begin{equation}
\begin{split}
&{\mathcal{P}}_{md}  = \mathcal{P}(H_0|H_1) = \mathcal{P}(TS^*<\epsilon|E_j) \\
& =\sum_{j=1}^{N} \sum_{i=1}^{M} \bigg[ Q(\frac{\Psi_i - \Psi_j - \epsilon}{\sigma}) - Q(\frac{\Psi_i - \Psi_j + \epsilon}{\sigma}) \bigg] \frac{\pi (j)}{M}
\end{split}
\end{equation}
where $\pi (j)$ is the prior probability of impersonator node $E_j$. 
%$\alpha_{ij}\in(0,1)$ is the fraction of time slots which are originally dedicated to legal follower node $F_i$ but are found idle and thus utilized by illegitimate node (impersonator node) $E_j$.

Since the probability of missed detection is a random variable, so the expected value $\bar{\mathcal{P}}_{md}:=\mathbb{E}(\mathcal{P}_{MD})$ is as follows:
\begin{equation} 
\begin{split}
&\bar{\mathcal{P}}_{md}  =\sum_{j=1}^N \frac{1}{\Delta}\pi (j). \\
& \resizebox{.5 \textwidth}{!}{$\bigg( \bigintsss_{\Psi_{min}}^{\Psi_{max}} \sum_{i=1}^M Q(\frac{\Psi_i - \Psi_j^{(E)} - \epsilon}{\sigma})  - Q(\frac{\Psi_i - \Psi_j^{(E)} + \epsilon}{\sigma}) d\Psi_j^{(E)} \bigg)$} \\
& =\sum_{j=1}^N \frac{1}{\Delta}\pi (j). \\
&\resizebox{0.5 \textwidth}{!}{$\bigg( \bigintsss_{\Psi_{min}}^{\Psi_{max}} \sum_{i=1}^M Q(\frac{\Psi_i - \Psi^{(E)} - \epsilon}{\sigma}) - Q(\frac{\Psi_i - \Psi^{(E)} + \epsilon}{\sigma}) d\Psi^{(E)} \bigg)$}
\end{split}
\end{equation}
where we have assumed that the unknown pathloss $\Psi_j\sim U(\Psi_{min},\Psi_{max})$ $\forall j$, and $\Delta=\Psi_{max}-\Psi_{min}$. 

Now, we investigate the authentication of the casted vote  by identifying the transmitter identity using the ML-based approach. 
The error probability of miss-classified node $\mathcal{P}_{mc}$ resulting from Eq. \ref{eq:ML-pl} is given as:    
\begin{equation}
\mathcal{P}_{mc} = \sum_{i=1}^M \mathcal{P}_{mc|i}.\pi(i)
\end{equation}
where $\mathcal{P}_{mc|i}$ is the probability that the leader notice that the vote is cast by follower $F_j$ but the vote is actually cast by follower $F_i$ where $i\neq j$.  For the hypothesis test of (\ref{eq:bht}), $\mathcal{P}_{mc|i}$ is given as:
\begin{equation}
\label{eq:pmc}
\mathcal{P}_{mc|i}=1-\bigg( Q(\frac{\tilde{\Psi}_{l,i}-\tilde{\Psi}_i}{\sigma}) - Q(\frac{\tilde{\Psi}_{u,i}-\tilde{\Psi}_i}{\sigma}) \bigg)
\end{equation}
where $\tilde{\Psi}_{l,i}=\frac{\tilde{\Psi}_{i-1}+\tilde{\Psi}_i}{2}$, $\tilde{\Psi}_{u,i}=\frac{\tilde{\Psi}_{i}+\tilde{\Psi}_{i+1}}{2}$. Additionally, $\mathbf{\tilde{\Psi}}=\{\tilde{\Psi}_{1},...,\tilde{\Psi}_{M}\}=\text{sort}(\mathbf{\Psi})$ where sort operation (.) sorts a vector in an increasing order. For the boundary cases, e.g., $i=1, i=M$, $\tilde{\Psi}_{l,1}=\Psi_{min}$, $\tilde{\Psi}_{l,M}=\Psi_{max}$ respectively.
\\ Note that the proposed mechanism will be executed at the leader node, which becomes uplink transmission according to the discussion of Section \ref{sec:Jamming}. For the downlink, the mechanism will be executed at followers having a single ground truth of the leader node. In this case, we will have two error probabilities (i.e., false alarm and missed detection) with a kind of similar error expressions given above (i.e., except summation for $N$ legitimate nodes). We omit the discussion of it for the sake of brevity.


==> Figures/sec3.tex <==

 \section{Results And Discussions}
 \label{sec:RESULTS}
We use MATLAB $2019a$ for simulations. The important simulation parameters for generated figures are mentioned in TABLE \ref{tb:1}, unless otherwise stated. 

 \begin{table}[ht]
 \begin{center}
      \begin{tabular}{ |p{4cm}|p{4cm}| }
 \hline
 Parameters& Configuration \\
 \hline
 $P_L$, $P_F$, $P_j$   & 30 dBm, 20 dBm, 10 dBm     \\
  \hline
 Pathloss exponent $\alpha$ &   $3$ \\
 \hline
  $\rho_F$ &  $15/\pi(500)^2 $  \\
 
  \hline
Area  & $\pi  (500m)^2$     \\
  \hline
  $M$, $N$  & $5$, $5$     \\
  \hline
\end{tabular}
 \end{center}
 \caption{Important simulation parameters}
 \label{tb:1}
  \end{table}
	\subsection{Coverage probability performance of the IoT blockchain network under jamming attack}
	
	Under a jamming attack, both legitimate and malicious nodes are deployed according to the PPP with $\rho_F$ intensity for legitimate nodes, and $\rho_J$ intensity for jammer/malicious nodes. The leader is placed at the origin. 
	
	Fig. \ref{fig:F1} presents the joint coverage probability for the  different SIR threshold values of $\beta$ (in dB) and intensity of jammers $\rho_J$. We observe that the transaction success rate (i.e., $\mathcal{P}_c$) declines as the SIR threshold increases. Fig. \ref{fig:F1} also reveals that increasing the jammer intensity severely degrades the transaction success rate.

\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm]{coverage_prob_1.eps}
    \caption{Transaction success probability vs SIR threshold $\beta$ for different jammers densities }
    \label{fig:F1}
\end{figure}

Fig. \ref{fig:F2} demonstrates the behavior of joint coverage probability against different radius values (i.e., effective area) of distributed jammers. Specifically, we set $\rho=\rho_J$, $z_1=0$ and vary $z_2$ from $0$ to $300$ by step of $20$. We observe that the increase in the effective jamming area of jammers causes low SIR values that lower the transaction success rate. We can also see the degradation in the performance of success rate with an increase in the intensity of jammers $\rho_J$.

\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm]{Distribution_Area_new_m2.eps}
    \caption{Transaction success probability vs effective jamming area  }
    \label{fig:F2}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Fig. \ref{fig:F3} presents the three computed coverage probabilities: UL, DL, and joint coverage probabilities against  the jamming distance (i.e., $z_1$) from the origin or leader. We vary $z_1$ from $0m$ to $300m$ and keep $z_2=z_1+50m$. In the upper two plots, the $\beta$ varies from $-30$ dB to $-20$ dB from left to right, and from $-10$ dB to $0$ dB in the lower two plots.  We notice that the effective jamming area (or can be thought as jammers) moves away from the leader, making the interference lower at the leader and resulting in higher UL coverage probability. Followers are deployed in $\pi (500m)^2$ area, so moving of jamming distance from the origin produces low DL coverage probability as jammers are getting close to followers. On the other hand, joint coverage probability first enhances and then goes down. Note that we need coverage probabilities greater than $0.5$ to achieve the consensus.


\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm]{jamming_distance.eps}
    \caption{Transaction success probability vs jamming distance}
    \label{fig:F3}
\end{figure}

\subsection{Authentication performance of the IoT blockchain network under impersonation attack}
We choose a realization of PPP for malicious and legitimate nodes where we have $M=N=5$ number of malicious and legitimate nodes. We set the link quality  as $LQ=1/\sigma^2$, which means that more uncertainty in the estimation/noise implies poor link quality and vice versa. 
We plot the error probabilities (false alarm, missed detection, and miss classification) as  functions of  $LQ$ (in dB) in Fig. \ref{fig:F5}.  We observe from this figure that pathloss can be exploited to counter impersonation attacks in wireless blockchain networks. A designed parameter $\epsilon$ can be set for the desired level of security. We observe that we can not minimize both errors for a given link quality simultaneously. In other words, increasing $\epsilon$ improves false alarm but degrades missed detection. The lower plot  of Fig. \ref{fig:F5} shows the miss classification error against link quality and it demonstrates that it is not a  function of   $\epsilon$, and that's why a single curve for all the three given choices of $\epsilon$.
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm,height=8cm]{ErrvsSNR_Raft_LQ.eps}
    \caption{Error Probabilities against $LQ$. From top to bottom: Probability of false alarm $P_{fa}$, probability of missed detection $P_{md}$ and probability of misclassification $P_{mc}$. }
    \label{fig:F5}
\end{figure}

Fig. \ref{fig:F6}
shows the Receiver Operating Characteristic (ROC) curves comprises two
error probabilities ($P_d$ and $P_{fa}$). where $P_d = 1 - P_{md}$ is the detection
probability is defined as the probability of correctly deciding malicious nodes. We sweep $P_{fa}$ from zero to one and find $P_{md}$ for different values of $1/\sigma^2$. As we can see improvements in link quality improves $P_d$. These curves can be used to set the system to the desired level of security where for a given link quality, one can find a value of false alarm for a desired value of detection.
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm,height=5cm]{ROCraft_LQ.eps}
    \caption{Receiver Operating Characteristic (ROC) curves: the probability of detection $P_d$ can be set to the desired level while compromising on probability of false alarm $P_{fa}$  }
    \label{fig:F6}
\end{figure}
